Explaining Classifiers Trained on Raw Hierarchical Multiple-Instance Data

Learning from raw data input, thus limiting the need for feature engineering, is a component of many successful applications of machine learning methods in various domains. While many problems naturally translate into a vector representation directly usable in standard classifiers, a number of data sources have the natural form of structured data interchange formats (e.g., security logs in JSON/XML format). Existing methods, such as in Hierarchical Multiple Instance Learning (HMIL), allow learning from such data in their raw form. However, the explanation of the classifiers trained on raw structured data remains largely unexplored. By treating these models as sub-set selections problems, we demonstrate how interpretable explanations, with favourable properties, can be generated using computationally efficient algorithms. We compare to an explanation technique adopted from graph neural networks showing an order of magnitude speed-up and higher-quality explanations.

==> json_example.tex <==
% \begin{wrapfigure}{r}{0.51\textwidth}
% \begin{minted}[fontsize=\tiny]{json}
% {"mac": "00:0e:58:fc:40:60",  
%  "ip": "192.168.254.24",
%  "services": [{"port": 1400, "protocol": "tcp"},
% 	       ...
%               {"port": 5353, "protocol": "udp"}],
%  "upnp": 
%   [{"model_name": "Sonos Play:3",
%      "model_description": "Sonos Play:3",
%      "manufacturer": "Sonos, Inc.",
%      "device_type": "urn:schemas-upnp-org:device:ZonePlayer:1",
%      "services": ["urn:upnp-org:serviceId:AlarmClock",
%                   "urn:upnp-org:serviceId:MusicServices",
%                         ...
% 	              "urn:tencent-com:serviceId:QPlay"]},
%     {"model_name": "Sonos Play:3",
%      "model_description": "Sonos Play:3 Media Server",
%      "manufacturer": "Sonos, Inc.",
%      "device_type": "urn:schemas-upnp-org:device:MediaServer:1",
%      "services": ["urn:upnp-org:serviceId:ContentDirectory",
%                   "urn:upnp-org:serviceId:ConnectionManager"]},
%     ...
% \end{minted}
% \caption{A part of an example data sample.}\label{fig:json}
% \end{wrapfigure}


==> problem.tex <==
\section{Problem Definition}\label{sec:problem}

\todo[inline]{[VL] Since the example was moved to the introduction, this section can be removed in order to save space. The parts that should me moved elsewhere are: (1) Note on hierarchical structure (intro), (2) More details on schema (HMILL, experiments), (3) Consistency (intro)}

 %Note that while we use the problem of device identification as a running example, all the presented methods are completely generic and applicable to any tree-structured data.


\paragraph{Explanation of a classification.}
We focus on classification models, where the input is a tree-structured data sample and the output is one of a fixed sets of output classes. We seek an explanation in the form a \textbf{subset of the input sample}, i.e., a subset of keys-value pairs in property nodes and a subset of items in the list nodes. The subset should be as small as possible, while still classified by the explained model to the same class as the complete sample. A property we call \textbf{consistency}. We take the consistency as a hard constrain and try to minimize the size of the explanation measured in the number of leaf values in the explanation.

\todo[inline]{Explain  better why smaller explanations are preferable.}
\todo[inline]{Link to related work? E.g., the IBM result.}
